Asynchronous Graph Pattern Matching on Multiprocessor Systems

Pattern matching on large graphs is the foundation for a variety of application domains. Strict latency requirements and continuously increasing graph sizes demand the usage of highly parallel in-memory graph processing engines that need to consider non-uniform memory access (NUMA) and concurrency issues to scale up on modern multiprocessor systems. To tackle these aspects, graph partitioning becomes increasingly important. Hence, we present a technique to process graph pattern matching on NUMA systems in this paper. As a scalable pattern matching processing infrastructure, we leverage a data-oriented architecture that preserves data locality and minimizes concurrency-related bottlenecks on NUMA systems. We show in detail, how graph pattern matching can be asynchronously processed on a multiprocessor system.

==> NUMA.tex <==
\section{Graph Pattern Matching on NUMA Systems}
\label{sec:NUMA}

To scale up graph pattern matching on large multiprocessor systems, we employ an approach that is based on a \emph{data-oriented architecture (DORA)}~\cite{Pandis2010}, which is known for its superior scalability on NUMA systems~\cite{Kissinger2014}.
As illustrated on the right hand side of Figure~\ref{fig:dora}, the graph is implicitly split into a set of disjoint partitions.
Each partition is placed in the local memory of a specific processor that runs \emph{workers} on its local hardware threads.
These workers are limited to operate exclusively on local graph partitions and leverage a high-throughput message passing layer for the inevitable communication.
Only one worker is allowed to access a partition at a time to avoid costly fine-grained lockings of the data structures.
Consequently, the number of workers is limited to the available local hardware threads and the number of local partitions can be chosen arbitrarily.
An integral part of the message passing layer is the \emph{routing table}, which keeps track of the partitioning and thus, maps the \emph{partitioning criteria} (cf., Section~\ref{sec:Partitioning}) to the corresponding partition using a hash table.
The overall goal of this architecture is (1) to restrict the access of threads to data structures in the local main memory, (2) to reduce the necessity of locks or atomic instructions, and (3) to hide remote memory latency using the high-throughput message passing layer.

To actually process \emph{conjunctive queries} on such a data-oriented architecture, the \emph{edge predicates} -- CQs are consisting of -- are evaluated one after another.
Every time an edge predicate matches within a partition, a new message is generated by the worker thread to evaluate the successive edge predicate unless the predicate was the last one of the CQ.
These messages are either sent to a single partition (unicast) or to all partitions (broadcast) depending on the edge predicate and partitioning criterion. 
Due to the topology-driven nature of pattern matching and the comprehensive structure of graphs, the appropriate selection of a \emph{partitioning strategy} for a specific combination of query pattern and underlying graph is crucial for such an architecture as we will show throughout this paper.  


==> system.tex <==
\section{System Overview}
\label{sec:system}

\noindent As described in Section~\ref{sec:intro}, our system design targets multisocket NUMA systems. 
With the fading of Moore's Law, hardware vendors are installing an increasing number of processors in a system rather than using only a few processors with very high frequency. 
The resulting massive parallelism and the ever growing size of available main memory demands a specialized system design to exploit the full potential of such a NUMA system.
In this section, we want to describe the architecture of our system and which components are involved in the \emph{graph pattern matching} process.

\subsection{General Architecture}
\label{sec:sysOverview}

As previously stated, we focus on scale-up NUMA systems for graph processing, since basically all publicly available graph data sets fit into the main memory of such scale-up systems. 
A NUMA system consists of multiple CPUs, so called sockets, where either socket is directly connected to a local main memory. 
However, all sockets can access another processors main memory through a communication network which can get increasingly complex, the more CPUs are installed in the system.
These remote memory accesses are expensive compared to the local memory access and impose a performance bottleneck, if not handled properly.
To solve this issue, we employ a fine grained, \emph{data-oriented architecture~(DORA)} as a foundation for our processing engine. 
The general layout of our system is depicted in Figure~\ref{fig:dora_abstract}.

Data processing is performed by worker threads, which are bound to a core. If the socket, i.e. the CPU supports Simultaneous Multithreading (SMT), one processor chip can support multiple workers at once, i.e. it provides the system with multiple virtual cores.
Each worker is able to process one data partition at a time, as specified by DORA.
Additionally, a worker thread is restricted to only access data partitions which resides on its local main memory.
This design eliminates latency issues which arise from uncontrolled data placement and data access.
By limiting the remote memory accesses solely to the communication between the worker threads, we enable our system to easily scale up with the employed hardware.

\begin{figure}[t]
	\includegraphics[width=\textwidth]{DORA_abstract}
	\caption{data oriented architecture principle}
	\label{fig:dora_abstract}
\end{figure}

\subsection{Communication}
\label{sec:sysCommunication}
The communication between all worker threads is handled by a high performance message passing layer, as illustrated in Figure~\ref{fig:dora_abstract}.
Since each message basically represents a copy operation from one memory region to another one, we hide the resulting latency by employing batching of multiple messages as well as multiple buffers per worker.
Messages are unavoidable, since the DORA inherently requires the data to be partitioned among the memory regions. 
Due to this data partitioning, one worker is most likely to not find all results of a data request on local partitions.
In this case, it sends messages to all sockets, which own a data partition containing the relevant data.
To achieve that, we store data locality information in a global routing table.
The layout of the routing table is also crucial for the systems performance, as there are numerous ways to implement it.
One frequently used approach is the usage of hashing data to partitions.
The usage of a hash function completely eliminates structural overhead for the routing table, since the data location can be directly computed.
However, hashing is unable to exploit context information or relations between the stored data elements, which is important for efficient graph processing.
An alternative routing table implementation is for example a ranged partitioning, which stores data points of a certain data range per partition.
This limits the size of the routing table to the total number of partitions, since only the upper bounds of each data partition need to be stored.
The most overhead in terms of storage cost results from a one to one mapping of data points to partitions.
By storing the target partition for every data point, we are able to leverage all context information as well as relations between the data points.
However, the theoretically better data partitioning comes at the cost of high storage overhead, since the whole data set is basically replicated to the routing table.
